Oobleck: Resilient Distributed Training of Large Models Using Pipeline Templates

Oobleck enables resilient distributed training of large DNN models with guaranteed fault tolerance. It takes a planning-execution co-design approach, where it first generates a set of heterogeneous pipeline templates and instantiates at least $f+1$ logically equivalent pipeline replicas to tolerate any $f$ simultaneous failures. During execution, it relies on already-replicated model states across the replicas to provide fast recovery. Oobleck provably guarantees that some combination of the initially created pipeline templates can be used to cover all available resources after $f$ or fewer simultaneous failures, thereby avoiding resource idling at all times. Evaluation on large DNN models with billions of parameters shows that Oobleck provides consistently high throughput, and it outperforms state-of-the-art fault tolerance solutions like Bamboo and Varuna by up to $29.6x$.

==> discussion.tex <==
%-------------------------------------------------------------------------------
\section{Discussion}
\label{sec:discussion}
%-------------------------------------------------------------------------------

\subsection{Considering ZeRO and Fully Sharded Data Parallel (FSDP)}
\label{sec:zero}
Zero Redundancy Optimizer (ZeRO) data parallelism shards the model states and each GPU in a GPU group only has portion of model states, allowing very large model training with relatively fewer number of GPUs by removing model states redundancy~\cite{2020zero}.
Inspired by ZeRO, PyTorch community has implemented their own version of sharded data parallelism (FSDP) in PyTorch~\cite{2023fsdp}.
During every forward and backward pass, a GPU that has the sharded portion of the model to be trained broadcasts it to all GPUs in the same group.
They compute activation or gradients on the received model states with a different batch input and release the received model states.
Although each GPU computes the same model states with a different input like DP, we categorize ZeRO and FSDP as another type of TP because \circled{1} no GPU in the group has duplicated model states, and \circled{2} broadcasting model states has high network communication overheads that cannot be hidden, similar to TP.
Therefore, they can be used as an alternative of TP in \name.
